Extensions and Analysis of an Iterative Solution of the Helmholtz Equation via the Wave Equation

In this paper we extend analysis of the WaveHoltz iteration -- a time-domain iterative method for the solution of the Helmholtz equation. We expand the previous analysis of energy conserving problems and prove convergence of the WaveHoltz iteration for problems with impedance boundary conditions in a single spatial dimension. We then consider interior Dirichlet/Neumann problems with damping in any spatial dimension, and show that for a sufficient level of damping the WaveHoltz iteration converges in a number of iteration independent of the frequency. Finally, we present a discrete analysis of the WaveHoltz iteration for a family of higher order time-stepping schemes. We show that the fixed-point of the discrete WaveHoltz iteration converges to the discrete Helmholtz solution with the order of the time-stepper chosen. We present numerical examples and demonstrate that it is possible to completely remove time discretization error from the WaveHoltz solution through careful analysis of the discrete iteration together with updated quadrature formulas.

==> iteration.tex <==
%!TEX root = WaveHoltz.tex

\section{WaveHoltz: A New Method for Designing Scalable Parallel Helmholtz Solvers}
We consider the Helmholtz equation in a bounded open smooth
domain $\Omega$,
\begin{equation}
  \nabla\cdot(c^2(x)\nabla u) + \omega^2u = f(x),\qquad
  x\in \Omega, \label{eq:helm}
\end{equation}
with boundary condtions of the type
\begin{equation}
i\alpha\omega u + \beta(c^2(x)\vec{n}\cdot \nabla u)=0,
\quad \alpha^2+\beta^2=1,\quad
\qquad x\in \partial\Omega.
 \label{eq:helmbc}
\end{equation}
We assume $f\in L^2(\Omega)$ and that $c\in L^\infty(\Omega)$ with
the bounds $0< c_{\min}\leq c(x)\leq c_{\max}<\infty$ a.e. in $\Omega$.
Away from resonances, this ensures that there is 
a unique weak solution $u\in H^1(\Omega)$
to (\ref{eq:helm}).
Due to the boundary conditions $u$ is in general complex valued.

We first note that the function $w(t,x) := u(x) \exp(i\omega t)$
is a $T=2\pi/\omega$-periodic (in time) 
solution to the forced scalar wave equation
\begin{eqnarray}
&&  w_{tt} =   \nabla\cdot(c^2(x)\nabla w)
  - f(x) e^{i\omega t}, \quad x\in\Omega, \ \ 0 \le t \le T, \nonumber \\
&&  w(0,x) = v_0(x), \quad w_t(0,x) = v_1(x), \nonumber \\
&&  \alpha w_t +\beta(c^2(x)\vec{n}\cdot \nabla w)=0, \quad x\in\partial\Omega
, \label{eq:apa}
\end{eqnarray}
where $v_0=u$ and $v_1=i\omega u$.
Based on this observation, our approach is to find this $w$
instead of $u$. We could thus look for
initial data  $v_0$ and $v_1$ such that $w$ is a $T$-periodic solution
to (\ref{eq:apa}). 
However, there may be several such $w$, see \cite{grote2019controllability}, 
and we therefore impose
the alternative constraint that a certain time-average of $w$
should equal the initial data. 
More precisely, we introduce the
following operator acting on the initial data $v_0\in H^1(\Omega)$, $v_1\in L^2(\Omega)$,
\be\lbeq{filterstep_diss}
{\Pi} \left[
\begin{array}{c}
v_0\\
v_1 
\end{array}
\right] = \frac{2}{T}\int_0^{T}\left(\cos(\omega t)-\frac14\right) \left[
\begin{array}{c}
w(t,x)\\
w_t(t,x) 
\end{array}
\right] dt,\quad
T=\frac{2\pi}{\omega},
\ee
where $w(t,x)$ and its time derivative $w_t(t,x)$ satisfies the wave equation (\ref{eq:apa}) with initial data $v_0$ and $v_1$.
The result of $\Pi [v_0,\ v_1]^T$ can thus be seen as
a filtering in time 
of $w(\cdot,x)$
around the $\omega$-frequency.
We will further 
motivate the choice of time averaging in the analysis below.
By construction, the solution $u$ of Helmholtz now satisfies the equation
\begin{equation}\lbeq{iteration_eq}
\left[
\begin{array}{c}
u\\
i\omega u 
\end{array}
\right] = {\Pi} \left[
\begin{array}{c}
u\\
i\omega u 
\end{array}
\right].
\end{equation}
The WaveHoltz method then amounts to solving
this equation with the fixed point iteration
\begin{equation}\lbeq{iteration_diss}
\boxed{
\left[
\begin{array}{c}
v\\
v' 
\end{array}
\right]^{(n+1)} = {\Pi} \left[
\begin{array}{c}
v\\
v' 
\end{array}
\right]^{(n)}, \qquad \left[
\begin{array}{c}
v\\
v' 
\end{array}
\right]^{(0)} \equiv 0.
}
\end{equation}
Provided this iteration converges and the solution to \eq{iteration_eq}
is unique, we 
obtain the Helmholtz solution as
$u=\lim_{n\to\infty} v^n$.

\begin{remark}
Note that each iteration is inexpensive and that $T$ is reduced by the reciprocal of $\omega$ as $\omega$ grows. If we assume that the number of degrees of freedom in each dimension scales with $\omega$ and that we evolve the wave equation with an explicit method this means that the number of time-steps per iteration is independent of $\omega$. Also note that the iteration is trivial to implement (in parallel or serial) if there is already a time domain wave equation solver in place. The integral in the filtering is carried out independently for each degree of freedom and simply amounts to adding up a weighted  sum (e.g. a trapezoidal sum) of the solution one time-step at a time. Finally, note that WHI allows all the advanced techniques that have been developed for wave equations (e.g. local time-stepping, non-conforming discontinuous Galerkin finite elements $h$- and $p$-adaptivity etc.) can be transferred to the Helmholtz equation and other time harmonic problems.       
\end{remark}

\subsection{Iteration for the Energy Conserving Case} \label{sec:iteration}

Here we consider boundary conditions of either
Dirichlet ($\beta=0$) or Neumann ($\alpha=0$) type. 
This is typically
the most difficult case for iterative Helmholtz solvers
when $\Omega$ is bounded.
The
wave energy is preserved in time and certain $\omega$-frequencies
in Helmholtz are resonant, meaning they equal an eigenvalue
of the operator $-\nabla\cdot(c^2(x)\nabla)$. Moreover,
the limiting amplitude principle does not hold, and one
can thus not obtain the Helmholtz solution by solving the
wave equation over a long time interval.

We start by introducing a simplified iteration for this case.
With the given boundary conditions
the solution to Helmholtz will
be real valued, since
$f$ is a real valued function.
Without loss of generality, we may then take $w_t(0,x)=0$ and $w(t,x) = u(x) \cos(\omega t)$, since for a $T$-periodic real valued 
solution there is a time when $w_t(0,x)=0$. We choose that time as the initial time so that (\ref{eq:apa}) becomes
\begin{eqnarray}
&&  w_{tt} =   \nabla\cdot(c(x)^2\nabla w)
  - f(x) \cos(\omega t), \quad x\in\Omega, \ \ 0 \le t \le T, \nonumber \\
&&  w(0,x) = v(x), \quad w_t(0,x) \equiv 0, \nonumber \\
&&  \alpha w_t +\beta(c^2(x)\vec{n}\cdot \nabla w)=0, \quad x\in\partial\Omega.
    \label{eq:wave}
\end{eqnarray}
The simplified iteration is then defined as
\begin{equation}\lbeq{iteration}
\boxed{  v^{n+1} = \Pi v^{n}, \qquad v^{0}\equiv 0,} 
\end{equation}
where
\be\lbeq{filterstep}
  \Pi v = \frac{2}{T}\int_0^{T}\left(\cos(\omega t)-\frac14\right)w(t,x) dt,\qquad
  T=\frac{2\pi}{\omega},
\ee
with $w(t,x)$ solving the wave equation (\ref{eq:wave}) with initial data $v=v^{n}\in H^1(\Omega)$.
We now analyze this iteration.


%
%We now propose a symmetric positive definite fixed point iteration that can be used to construct highly scalable parallel solvers for Helmholtz type equations. 
%
%
%
%We analyze our iteration for the interior problem, which is typically
%the most difficult one for iterative Helmholtz solvers.
%We thus consider
%a problem in an open bounded domain $\Omega$ with Dirichlet boundary conditions on $\partial\Omega$. 
By the choice of boundary conditions the operator 
$-\nabla\cdot(c^2(x)\nabla)$ has a point spectrum with non-negative
eigenvalues. Denote those eigenmodes $(\lambda_j^2,\phi_j(x))$. We assume that the angular frequency $\omega$ is not a resonance, i.e. $\omega^2\neq \lambda_j^2$ for all $j$. The Helmholtz equation (\ref{eq:helm}) is then wellposed. 

We recall that for any $q\in L^2(\Omega)$ we can
expand
$$
  q(x) = \sum_{j=0}^\infty \hat{q}_j\phi_j(x),
$$
for some coefficients $\hat{q}_j$ and
$$
   ||q||_{L^2(\Omega)}^2 = \sum_{j=0}^\infty |\hat{q}_j|^2,\qquad
   c_{\min}^4||\nabla q||_{L^2(\Omega)}^2
\leq   \sum_{j=0}^\infty \lambda_j^2|\hat{q}_j|^2\leq 
      c_{\max}^4||\nabla q||_{L^2(\Omega)}^2.
$$
We start by
expanding the Helmholtz solution $u$, the initial data $v$ to the wave equation (\ref{eq:wave}), and the forcing $f$ in this way,
\[
  u(x) = \sum_{j=0}^\infty \hat{u}_j \phi_j(x), \ \ \ \  v(x) = \sum_{j=0}^\infty \hat{v}_j \phi_j(x), \ \ \ \    f(x) = \sum_{j=0}^\infty \hat{f}_j \phi_j(x).
\]
Then,
\[
-\lambda_j^2\hat{u}_j+\omega^2\hat{u}_j = \hat{f}_j \quad\Rightarrow\quad
\hat{u}_j = \frac{\hat{f}_j}{\omega^2-\lambda_j^2}.
\]
For the wave equation solution $w(t,x)$ with initial data $w=v$ and $w_t=0$ we have
\be
  w(t,x) = \sum_{j=0}^\infty \hat{w}_j(t) \phi_j(x),\qquad
  \hat{w}_j(t) 
  =\hat{u}_j\Bigl(\cos(\omega t) -\cos(\lambda_j t)\Bigr)
  + \hat{v}_j\cos(\lambda_j t). \label{eq:no_filter_yet}
\ee
The filtering step \eq{filterstep} then gives
$$
\Pi v = \sum_{j=0}^\infty \bar{v}_j \phi_j(x),\qquad
\bar{v}_j = \hat{u}_j(1-\beta(\lambda_j)) + \hat{v}_j\beta(\lambda_j), 
$$
where
\[
\beta(\lambda)
:= \frac{2}{T}\int_0^T \left(\cos(\omega t)-\frac14\right)\cos(\lambda t) dt.
 \]
Introducing the linear operator ${\mathcal S}:L^2(\Omega)\to L^2(\Omega)$,
\be\lbeq{Sdef}
 {\mathcal S} \sum_{j=0}^\infty \hat{u}_j \phi_j(x) := \sum_{j=0}^\infty \beta(\lambda_j)\hat{u}_j \phi_j(x),
\ee
we can write the iteration as
\begin{equation}
  v^{n+1} =\Pi v^n= {\mathcal S}(v^n-u)+u. \label{eq:Siter}
\end{equation}
The operator ${\mathcal S}$ is self-adjoint and has the same eigenfunctions $\phi_j(x)$ as $-\nabla\cdot(c^2(x)\nabla)$ but with the (real)
eigenvalues  $\beta(\lambda_j)$. 
The convergence properties of the iteration depend on these
eigenvalues and
it is therefore of interest to study the 
range of the filter transfer function $\beta$.
Figure~\ref{fig:beta} shows a plot of $\beta$ which indicates
that the eigenvalues of $ {\mathcal S}$ 
are inside the unit interval, with 
a few of them being close to 1 (when $\lambda_j\approx \omega$), and
most of them being close to zero (when $\lambda_j\gg \omega$). 
In the appendix we show the following lemma about $\beta$.
\begin{figure}[]
\graphicspath{{figures/}}
\begin{center}
\includegraphics[width=0.48\textwidth]{betapic}
\caption{The filter transfer function $\beta$ for $\omega=10$.
\label{fig:beta}}
\end{center}
\end{figure}
\begin{lemma}\lblem{filterlemma}
The filter transfer function $\beta$ satisfies $\beta(\omega)=1$ and
\begin{align*}\lbeq{betabound}
0 \leq    \beta(\lambda) &\leq
   1 - \frac12 \left(\frac{\lambda-\omega}{\omega}\right)^2, 
   &{\rm when}\  \left|\frac{\lambda-\omega}{\omega}\right|\leq \frac12,\\
   |\beta(\lambda)| &\leq \frac12,
   &{\rm when}\  \left|\frac{\lambda-\omega}{\omega}\right|\geq \frac12,\\
   |\beta(\lambda)| & \leq 
   b_0 \frac{\omega}{\lambda-\omega}, &{\rm when}\  \lambda>\omega.
\end{align*}
where  $b_0 = \frac{3}{4\pi}$.
Moreover, 
close to $\omega$ we have the local expansion
\be\lbeq{locexp}
\beta(\omega+r) = 1- b_1 \left(\frac{r}{\omega}\right)^2 +
R(r/\omega)\left(\frac{r}{\omega}\right)^3 ,\qquad b_1 = \frac{2\pi^2}{3}-\frac14\approx 6.33,\quad
||R||_\infty\leq \frac{10\,\pi^{3}}{9}.
\ee
\end{lemma}
\begin{remark}
It is easy to see that $\beta(\omega)=1$ for any
constant besides $1/4$. The particular choice $1/4$ is made to ensure
that $\beta'(\omega)=0$, which is necessary to keep $\beta\leq 1$ in a neighborhood of $\omega$.
We explore other possibilities in Section~\ref{sec:time_dep_fil}.
\end{remark}


From this lemma we can derive some results for the 
operator ${\mathcal S}$. To do this we first quantify
the non-resonance condition. We let
\[
 \delta_j =\frac{\lambda_j-\omega}{\omega},
\]
be the relative size of the gap between $\lambda_j$ and the Helmholtz frequency, and then denote the smallest gap (in magnitude) by $\delta$,
$$
   \delta =\delta_{j^*},\qquad 
   j^*={\rm argmin}_j |\delta_j|.
$$ 
Then we have
\begin{lemma}\lblem{Slemma}
Suppose $\delta>0$. The spectral radius $\rho$ of ${\mathcal S}$
is strictly less than one, and for small $\delta$,
\be\lbeq{rhoest}
  \rho = 1-b_1\delta^2 + O(\delta^3),
\ee
with $b_1$ as in \lem{filterlemma}. Moreover,
${\mathcal S}$ is a bounded linear map from
$L^2(\Omega)$ to $H^1(\Omega)$.
\end{lemma}
\begin{proof}
From \lem{filterlemma} we get
$$
   \rho = \sup_j |\beta(\lambda_j)|
   \leq \sup_j\max\left(1-\frac12\delta_j^2,\ \frac12\right)
   \leq \max\left(1-\frac12\delta^2,\ \frac12\right)<1.
$$ 
For the more precise estimate when $\delta$ is small
we will use \eq{locexp}. 
Since $1>\rho\geq\beta(\omega+\omega\delta)\to 1$ as $\delta\to 0$,
we can assume that
$\rho> 1-\eta^2/2$, with $\eta:=b_1/2||R||_\infty$,
for small enough $\delta$.
Then, since $|\beta(\omega+\omega\delta_j)|\leq 1-\eta^2/2$
for $|\delta_j|>\eta$ 
by \lem{filterlemma}, we have
$$
   \rho    =
   \sup_{|\delta_j|\leq \eta} \beta(\omega+\omega\delta_j) = 
   \beta(\omega+\omega\delta_{k^*}),
$$ 
for some $k^*$ with $|\delta_{k^*}|\leq \eta$. 
If $\delta_{k^*}=\delta_{j^*}$ (where $\delta=|\delta_{j^*}|$)
then \eq{locexp} gives \eq{rhoest}.
If not, we have
$\eta\geq |\delta_{k^*}|\geq\delta$ and by \lem{filterlemma}
$$
  0\leq \beta(\omega+\omega\delta_{k^*})-
  \beta(\omega+\omega\delta_{j^*})
  =-b_1(\delta^2_{k^*}-\delta^2)
  +R(\delta_{k^*})\delta^3_{k^*}
  -R(\delta_{j^*})\delta^3_{j^*}
  \leq
  -b_1(\delta^2_{k^*}-\delta^2)+
   \frac{b_1}2(\delta^2_{k^*}+\delta^2),
$$
which implies that $\delta_k^2\leq 3\delta^2$ and therefore
$$
{\rho} = 
1-b_1\delta_{k^*}^2 + O(\delta_{k^*}^3)
=
1-b_1\delta^2 + 
b_1(\delta^2-\delta_{k^*}^2)+
O(\delta_{k^*}^3)
=
1-b_1\delta^2 + 
O(\delta_{k^*}^3+\delta^3)
=
1-b_1\delta^2 + 
O(\delta^3).
$$
This shows \eq{rhoest}.
For the second statement, we note first that by \eq{betabound},
$$
  |\lambda_j\beta(\lambda_j)|\leq 
  \omega\ \begin{cases}
   1, & \lambda_j\leq \omega,\\
   \frac{b_0\lambda_j}{\lambda_j-\omega}, & \lambda_j> \omega,
  \end{cases}
  \ \ 
=  \omega\ \begin{cases}
   1, & \lambda_j\leq \omega,\\
   b_0(1+1/\delta_j), & \lambda_j> \omega,
  \end{cases}\ \ 
  \leq \omega \min(1,b_0(1+1/|\delta|))=:D.
$$
Suppose now that $g\in L^2(\Omega)$ and
$$
  g(x) = \sum_{j=0}^\infty \hat{g}_j \phi_j(x).
$$
Then
\begin{align*}
   ||{\mathcal S}g||_{H^1(\Omega)}^2
   &\leq \sum_{j=0}^\infty |\beta(\lambda_j)|^2|\hat{g}_j|^2 +
   \sum_{j=0}^\infty\frac{\lambda_j^2}{c^4_{\min}}|\beta(\lambda_j)|^2|\hat{g}_j|^2
   \leq 
   \left(1 +
   \frac{D^2}{c^4_{\min}}\right)
   \sum_{j=0}^\infty |\hat{g}_j|^2=
   \left(1 +
   \frac{D^2}{c^4_{\min}}\right)
   ||g||_{L^2(\Omega)}^2.
\end{align*}
This proves the lemma.
\end{proof}
Letting $e^n:=u-v^n$ we can rearrange
(\ref{eq:Siter}) and obtain
$$
  e^{n+1}=  {\mathcal S}e^n\quad\Rightarrow\quad
  ||e^{n+1}||_{L^2(\Omega)}\leq \rho
  ||e^{n}||_{L^2(\Omega)}
  \quad\Rightarrow\quad ||e^{n}||_{L^2(\Omega)}
  \leq \rho^n ||e^{0}||_{L^2(\Omega)}\to 0,
$$
which shows that $v^n$ converges to $u$ in $L^2$. 
By \lem{Slemma} all iterates $v^n\in H^1(\Omega)$ since
$v^0=0$. We can therefore also get convergence in $H^1$.
Let 
$$
e^n(x) = 
\sum_{j=0}^\infty \hat{e}^{n}_j\phi_j(x),
$$
and consider similarly
\begin{align*}
\sum_{j=0}^\infty |\hat{e}^{n+1}_j|^2\lambda_j^2
&=
\sum_{j=0}^\infty \beta(\lambda_j)^2|\hat{e}^{n}_j|^2\lambda_j^2
\leq \rho^2\sum_{j=0}^\infty |\hat{e}^{n}_j|^2\lambda_j^2
\quad\Rightarrow\quad\\
||\nabla e^n||^2_{L^2(\Omega)}&\leq 
\frac{1}{c_{\min}^4}
\sum_{j=0}^\infty |\hat{e}^{n}_j|^2\lambda_j^2
\leq
\frac{\rho^{2n}}{c_{\min}^4}
\sum_{j=0}^\infty |\hat{e}^{0}_j|^2\lambda_j^2
\leq
\rho^{2n}\frac{c_{\max}^4}{c_{\min}^4}
||\nabla e^0||^2_{L^2(\Omega)}\to 0.
\end{align*}
We conclude that the iteration converges 
in $H^1$
with convergence rate $\rho$.
By \lem{filterlemma} we have
$\rho\sim 1-6.33\delta^2$ and, 
not surprisingly, the smallest gap, $\delta$, determines the convergence factor. 
We have thus showed
\begin{theorem}
The iteration in \eq{iteration} and \eq{filterstep} converges
in $H^1(\Omega)$
for the Dirichlet and Neumann problems
away from resonances
to the solution of the Helmholtz equation 
(\ref{eq:helm}). The convergence rate is $1-O(\delta^2)$,
where $\delta$ is the minimum gap between $\omega$ and 
the eigenvalues of $-\nabla\cdot(c^2(x)\nabla)$.
\end{theorem}
As discussed in the introduction,
the dependence of the convergence rate
on $\omega$ is often of interest. For the energy conserving
case, however,
this question is ambiguous as the problem
is not well-defined for all $\omega$. As soon as $\omega=\lambda_j$
there are either no or an infinite number of solutions.
In higher dimensions,
the eigenvalues $\lambda_j$ get denser as $j$ increases, meaning
that in general the problem will be closer and closer to resonance
as $\omega$ grows. Therefore, solving
the interior undamped Helmholtz equation for
high frequencies,
with pure Dirichlet or Neumann 
boundary conditions, may not be of great practical interest.

Nevertheless, we can make the following analysis. By the work of Weyl \cite{weyl:11} we know  that the eigenvalues grow asymptotically as $\lambda_j \sim j^{1/d}$ in $d$ dimensions. The average minimum gap $\delta$ when $\omega\approx \lambda_j$ is then 
$$
\delta \approx
\frac{1}{\lambda_{j+1}-\lambda_{j}}\int_{\lambda_j}^{\lambda_{j+1}}
\frac{\min(\lambda-\lambda_j,\lambda_{j+1}-\lambda)}{\omega}d\lambda
 =\frac{\lambda_{j+1}-\lambda_j}{4\omega}\sim \frac{(j+1)^{1/d}-j^{1/d}}{\omega}
\approx \frac{j^{1/d-1}}{d\omega}\sim
\frac{\omega^{1-d}}{\omega}\sim \omega^{-d}.
$$
When the convergence rate is $1-O(\delta^2)$, the number
iterations to achieve a fixed accuracy grows as $O(1/\delta^2)$.
This shows that the number of iterations 
would grow at the unacceptable rate $\omega^{2d}$
for the iteration. 


Fortunately, one can accelerate the convergence by using the conjugate gradient method in the energy conserving case and with any other Krylov method in the general case. The linear system that we actually want to solve is 
$$
(I- {\mathcal S})v =:  {\mathcal A}v = b := \Pi 0.
$$
Moreover, with $b=\Pi 0$ pre-computed we can easily evaluate the action of ${\mathcal A}$ 
at the cost of a single wave solve. Precisely, since $ {\mathcal A}v=v-\Pi v+b$ we simply carry out the evaluation of ${\mathcal A}v$
by evolving the wave equation for one period in time with $v$ as the initial data and then subtract the filtered solution from the sum of the initial data and the right hand side $b$.


%\daniel{}{}{Can you maybe expand this a bit more, with one or two sentences? It is an important point that the action of ${\mathcal A}$ can be evaluated cheaply, but it is a bit hidden away here. / Olof }

The operator ${\mathcal A}$ is self adjoint and positive, since 
$-1/2<\beta(\lambda_j)<1$, which implies that the eigenvalues of ${\mathcal A}$ lie in the interval $(0,3/2)$. The condition number of ${\mathcal A}$ is of the same order as $1-\rho$, where $\rho$ is the spectral radius of ${\mathcal S}$, i.e. 
by the simple analysis above,
${\rm cond}({\mathcal A})\sim \omega^{2d}$. 
If this system is solved using the (\emph{unconditioned}) conjugate gradient method the convergence rate is $1-1/\sqrt{{\rm cond}({\mathcal A})}\sim 1-1/\omega^d$, \cite{bjorck2015numerical}. Thus, then the method just requires $\sim \omega^d$ iterations for fixed accuracy. 

\begin{remark}
The operator $ {\mathcal A}$ is self-adjoint and coercive
when $\delta>0$ 
since
$$
   \ip{{\mathcal A}u,u} = \ip{(I-{\mathcal S})u,u} = 
\sum_{j=0}^\infty (1-\beta(\lambda_j))|\hat{u}_j|^2
\geq (1-\rho)||u||^2.
$$
This should be contrasted with
the original indefinite Helmholtz problem, which is not coercive. In fact, the eigenvalues satisfy the simple relation $\lambda_{\rm WHI} = 1-\beta(\lambda_{\rm Helmholtz} + \omega)$ > 0. The two formulations are however mathematically equivalent for the interior
Dirichlet and Neumann problems away from resonances,
as the analysis above shows. 

The coercivity also implies that the solution to
\eq{iteration_eq} for the simplified iteration
is unique since $w=\Pi w$ is equivalent to
${\mathcal A}(w-u)=0$.
\end{remark}


\begin{remark}
A discretization would have approximately a fixed number
of grid points per wavelength, leading to a (sparse) matrix
of size $N\times N$ with $N\sim \omega^d$. Hence, the number
of iterations for WHI would be $O(N^2)$
and the total cost $O(N^3)$ since each iteration costs $O(N)$.
This should be compared with a direct solution method which
is better than $O(N^3)$ when the matrix is sparse. %\ldots \daniel{}{}{ADD SOMETHING HERE???}
\end{remark}

\begin{remark}
In the Krylov accelerated case this analysis suggests that the number of iterations would now be $O(N)$ and the total cost $O(N^2)$. However, in the experiments below we observe slightly better complexity for interior problems and significantly better complexity for open problems. In fact, for the open problems we find that, in both two and three dimensions, the number of iterations scale as $\sim \omega$ which is the required number of iterations  for the information to travel through the domain.    
\end{remark}

%\begin{remark}
%\daniel{Equation (\ref{eq:no_filter_yet}) clearly illustrates the problems of not filtering: First, many irrelevant frequencies (multiples of $\omega/2$) are not damped at all. Second, without filtering there may be multiple solutions to $\Pi u=u$ if $n \omega$ is an eigenvalue (this may happen even if omega is not an eigenvalue). Indeed, in higher dimensions this is likely to happen as the eigenvalues get denser as they grow.}{ADDED}{}
%\end{remark}

==> theory_1D_Impedance.tex <==
%!TEX root = WaveHoltz2.tex
\subsection{Convergence in the Non-Energy Conserving Case}
With Theorem~\ref{thm::FirstOrderConv} providing convergence of the general 
WaveHoltz iteration in the energy-conserving case, we turn towards proving 
convergence for problems with impedance boundary conditions.
For simplicity, we prove convergence in a single spatial 
dimension as it is possible for the following proof technique 
to be extended to higher dimensions for particular 
problems. Consider now the following Helmholtz problem with impedance boundary conditions
  \begin{align*}
    \left[c^2(x) u'(x)\right]' & + \omega^2 u(x) = f(x), \quad a_0 \le x \le b_0, \\
    i \alpha \omega u(a_0) & - \beta(c(x) u_x(a_0)) = 0, \\ 
    i \alpha \omega u(b_0) & + \beta(c(x) u_x(b_0)) = 0,
  \end{align*}
where $\alpha, \, \beta \ne 0$. Here we assume $1/c \in L^1_{\text{loc}}([a_0,b_0])$ and 
that $c(a) = c_a$, $c(b) = c_b$ where $c$ is constant near the endpoints. 
We reformulate this in the time domain as 
  \begin{eqnarray*}
    &&  w_{tt} =   \frac{\partial}{\partial x} \left[c^2(x) \frac{\partial}{\partial x}w\right]
      - f(x) e^{i \omega t}, \quad a_0\le x \le b_0, \ \ 0 \le \tau \le T, \nonumber \\
    &&  w(0,x) = v_0(x), \quad w_t(0,x) = v_1(x), \nonumber \\
    &&  \alpha w_t(\tau,a_0) -\beta(c(x) w_x(\tau,a_0))=0,\\
    &&  \alpha w_t(\tau,b_0) +\beta(c(x) w_x(\tau,b_0))=0.
  \end{eqnarray*}
In general, the solution of the above equation will yield complex-valued solutions 
and so we take the real part of the 
equation as shown earlier and use the general iteration \eqref{eqn::Iteration}. 
Note that in $1$D  the impedance boundary conditions with $\alpha = \beta = 1/\sqrt{2}$ are 
equivalent to outflow/radiation conditions.
If $\alpha \ne \beta$ with $\alpha, \, \beta \ne 0$, then in addition to outgoing waves at the boundary
there will be reflections due to the impedance boundary condition.
In either case, if we let $a < a_0 - c_aT/2$ and $b > b_0 + c_bT/2$, the above problem is equivalent to 
  \begin{eqnarray}\label{eqn::ExtTD}
    &&  w_{tt} =   \frac{\partial}{\partial x} \left[\tilde{c}^2(x) \frac{\partial}{\partial x}w\right]
      - \text{Re}\{f(x) e^{-i\omega t}\}, \quad a\le x \le b, \ \ 0 \le \tau \le T, \nonumber \\
    &&  w(0,x) = \tilde{v}_0(x), \quad w_t(0,x) = \tilde{v}_1(x), \nonumber \\
    &&  w(\tau,a) = w(\tau,b))=0,
  \end{eqnarray}
where $\tilde{v}_0, \tilde{v}_1$ are zero extensions of $v_0,v_1$, and 
$\tilde{c}$ is the extension (with $\gamma = \alpha/\beta$)
\begin{align*}
\tilde{c}(x) = 
  \begin{cases}
    \gamma c_a, & a \le x < a_0, \\
    c(x), & a_0 \le x \le b_0, \\
    \gamma c_b, & b_0 < x \le b.
  \end{cases}
\end{align*}
That is, we extend the domain such that traveling waves may reflect 
off of the Dirichlet boundary but not re-enter the domain of interest,
$a_0 \le x \le b_0$, within a period $T$. The iteration then becomes $\tilde{\Pi} = P \Pi$ 
where $P$ is a projection operator onto the initial interval, i.e.
$P v(x) = v(x)|_{a_0\le x \le b_0}$.
Clearly $P$ is an orthogonal projection so that  
  \begin{align*}
    \|\tilde{\Pi} \tilde{v}\|_{L^2([a,b])} \le \|\Pi \tilde{v}\|_{L^2([a,b])},
  \end{align*}
and then we may apply Theorem \ref{thm::FirstOrderConv} to obtain convergence 
if it can be guaranteed that $\omega^2 \ne \lambda_j^2$ where 
$\lambda_j^2$ is an eigenvalue of the operator $-\partial_x(\tilde c^2(x) \partial_x)$. 

In order to obtain convergence in the case of impedance boundary conditions, 
results on the continuity of eigenvalues of the Laplacian from \cite{kong1996eigenvalues}
will be used. We present the framework of \cite{kong1996eigenvalues} in its full
generality and consider the following differential equation
  \begin{align}\label{eqn::SL_eq}
    -(py')' + qy = \lambda w y, \quad x \in (a',b'), \quad -\infty \leq a' < b' \le \infty, \quad \lambda \in \mathbb{R},
  \end{align}
where 
  \begin{align}\label{eqn::SL_conds}
    p,\,q,\,w: \, (a',b') \rightarrow \mathbb{R}, \quad 1/p,\, q,\, w \in L^1_{\text{loc}}(a',b'), \quad w>0 \, \text{ a.e. on } (a',b').
  \end{align}
Let
  \begin{align}\label{eqn::SL_Int}
    I=[a,b], \quad a'<a<b<b',
  \end{align}
and consider the boundary condition
  \begin{align}\label{eqn::SL_BC}
    A
    \begin{pmatrix}
    y(a) \\ (py')(a)  
    \end{pmatrix}
    +
    B
    \begin{pmatrix}
    y(b) \\ (py')(b),
    \end{pmatrix}
    =
    \begin{pmatrix}
    0 \\ 0
    \end{pmatrix}
  \end{align}
where the matrices $A, B \in \mathbb{C}^{2\times 2}$ are such that $(A | B) \in \mathbb{C}^{2\times 4}$ has full rank and $AEA^* = BEB^*$ with 
  \begin{align*}
    E = \begin{pmatrix}0 & -1\\1 & 0\end{pmatrix}.
  \end{align*}
We will be particularly interested in the case of Dirichlet boundary conditions for which $A=B$ with $A$ the 
matrix of zeros with a single non-zero entry $A_{11} = 1$. In this case, the Sturm-Liouville (SL) problem
\eqref{eqn::SL_eq}-\eqref{eqn::SL_conds} is such that all eigenvalues are real, simple, and can be ordered to satisfy
  \begin{align*}
    -\infty < 0 < \lambda^2_0 < \lambda^2_1 < \lambda^2_2 < \dots; \quad \lim_{n\rightarrow \infty} \lambda^2_n = + \infty.
  \end{align*}
For the particular case where $p=c$, $q=0$, and $w=1$, we immediately have that the eigenvalues of the Laplacian are
countable.

Let $\boldsymbol{\Omega} = \{\boldsymbol{\omega} = (a,b,A,B,1/p,q,w)\}$ such that \eqref{eqn::SL_conds}, 
\eqref{eqn::SL_Int}, and \eqref{eqn::SL_BC} hold. Letting $\|\cdot\|$ be any fixed matrix norm, then 
the following theorem from \cite{kong1996eigenvalues} holds.

\begin{theorem}[Kong \& Zettle]\label{thm:TheoremKong}
  Let $\boldsymbol{\omega}_0 = (a_0,b_0,A_0,B_0,1/p_0,q_0,w_0) \in \boldsymbol{\Omega}$. Let $\lambda = \lambda(\boldsymbol{\omega})$ be an eigenvalue of the SL problem \eqref{eqn::SL_eq}-\eqref{eqn::SL_BC} with $p=\tilde{c}$, $q=0$, and $w=1$. Then $\lambda$ is continuous at $\boldsymbol{\omega}_0$. That is, given any $\epsilon>0$, there exists a $\delta > 0$ such that if $\boldsymbol{\omega} \in \boldsymbol{\Omega}$ satisfies
    \begin{align*} 
       \|\boldsymbol{\omega} - \boldsymbol{\omega}_0\| = |a-a_0| + |b-b_0| + \|A-A_0\| + \|B-B_0\| + \int_{a'}^{b'} \left(|\widetilde{1/p} - \widetilde{1/p_0}| + |\tilde q - \tilde{q_0}| +  |\tilde w - \tilde{w_0}| \right) < \delta,
     \end{align*} 
then
  \begin{align*}
    |\lambda(\boldsymbol{\omega}) = \lambda(\boldsymbol{\omega}_0)| < \epsilon.
  \end{align*}
\end{theorem}

That is, the eigenvalues of the SL problem are continuous functions of the parameters of the problem including the coefficients, endpoints, and boundary conditions. As a consequence of Theorem~\ref{thm:TheoremKong}, we have
\begin{lemma}\label{lemma:Impedance}
  Suppose $\tilde{c} \ge 0$ a.e., fix $a$, and consider the Dirichlet eigenvalues $\lambda^2_n(\tilde{b})$ for $\tilde{b} \in (b_0 + c_bT/2,r)$ where $r>b_0 + c_bT/2$. Then there exists an endpoint $b \in (b_0 + c_bT/2,r)$ such that $\omega^2 \ne \lambda^2_n(b)$.  
\end{lemma}
\begin{proof}
  Suppose that there is no $b \in (b_0 + c_bT/2,r)$ such that $\omega^2 \ne \lambda^2_n$ where $n \in \mathbb{N}_0$ and $\lambda^2_n \equiv \lambda^2_n(b)$. Then for every $\delta > 0$ we have that $\omega^2 = \lambda^2_m(b + \delta)$ for some $m \in \mathbb{N}_0$. It follows that there must be an uncountable number of $\lambda^2_n$ for every $b \in (b_0 + c_bT/2,r)$ which contradicts the countability of the point spectrum of $-\partial_x(\tilde{c}^2(x) \partial_x)$.
\end{proof}

From this we can prove the following theorem.
\begin{theorem}\label{thm:TheoremOutflow}
  The iteration \eqref{eqn::Iteration} and \eq{filterstep} converges in $H^1 \times L^2$ for the Helmholtz problem with impedance boundary conditions to the solution of the 
  Helmholtz equation \eqref{eq::helm}-\eqref{eq::helmbc}.
\end{theorem}
\begin{proof}
  By Lemma \ref{lemma:Impedance}, there exists an extended wave equation \eqref{eqn::ExtTD} 
  with Dirichlet boundary conditions such that the eigenvalues of the extended domain
  Laplacian, $-\partial_x(\tilde{c}^2 w_x)$, are not in resonance. By \ref{thm::FirstOrderConv}
  the iteration \eqref{eqn::Iteration} converges in $H^1\times L^2$ with a 
  convergence rate of $1 - \mathcal{O}(\delta^2)$ where
  $\delta$ is the minimum gap between $\omega$ and the eigenvalues of the extended Laplacian.
\end{proof}

\begin{remark}
  The above analysis is for a single spatial dimension, but we note that it in certain 
  situations it may be extended to higher dimensions. For instance, interior impedance problems 
  with constant coefficients may be extended by an appropriate enclosing box from which the above arguments 
  can give convergence. In general, it is difficult to prove convergence in higher dimensions as 
  care needs to be taken to make appropriate wavespeed extensions that avoid reflections due to potentially
  discontinuous wavespeeds close to boundaries with impedance conditions.
\end{remark}

==> theory_Rn.tex <==
%!TEX root = WaveHoltz2.tex
\subsection{Theory in 2D and 3D}
Analysis for higher dimensional problems. Perhaps we need to make the following assumptions:
	\begin{itemize}
		\item Constant coefficients.
		\item Perfect ABC's.
		\item Regularity/Smoothness of problem domain $\Omega$ and its boundary.
	\end{itemize}
Using the same idea of enclosing the domain of interest in a larger box with Dirichlet 
(or possibly some other convenient) boundary conditions, we have a few options for 
bounding domains. Some information:
	\begin{enumerate}
		\item In general, we should expect eigenvalues that are no longer simple.
		\item Consider a bounding box, $\Omega = [0,\ell] \times [0,L]$. 
			\begin{enumerate}
				\item If $\ell/L$ is rational the eigenvalues may be degenerate.
				\item In the constant coefficient case, the eigenvalues are 
					\begin{align*}
						\lambda^2_{n,m} = \pi^2\left(\frac{m^2}{L^2} + \frac{n^2}{\ell^2}\right), m,n \ge 1,
					\end{align*}
			\end{enumerate}
		\item If we index the eigenvalues monotonically, then for $\lambda_n$ the corresponding eigenfunction
		$u_n$ has at most $n$ nodal regions.
		\item The restriction of $u_n$ to a nodal region gives that its first eigenvalue is $\lambda_n$.
		\item Faber-Krahn Inequality:
			\begin{align*}
				\lambda_1^D \ge \left(\frac{\omega_d}{\mu_d(\Omega)}\right)^{2/d}(j_{d/2-1,1})^2,
			\end{align*}
		where $j_{\nu,1}$ is the first positive zero of $J_\nu(z)$, $\mu_d(\Omega)$ is the measure of $\Omega$, and $\omega_d$ is the volume of the unit ball in $d$ dimensions. This in conjunction with the above item can be combined to get a lower bound on a given eigenvalue (given that something is known about the nodal region of $u_n$).
			\begin{enumerate}
				\item Are the nodal regions in the constant coefficient case an equal partitioning of $\Omega$?
			\end{enumerate}
		\item If we are interested in, say, the gap between $\lambda^2_m$ and $\lambda^2_n$ for not necessarily consecutive eigenvalues, there is an estimate (Grebenkov, Nguyen pg. 616) of the \textit{fundamental gap} in the constant coefficient Dirichlet case
			\begin{align*}
				\frac{d\pi^2}{\rho^2} \ge \lambda^2_2 - \lambda^2_1 \ge \frac{\pi^2}{4\delta^2},
			\end{align*}
		where $\delta$ is the diameter of $\Omega$ and $\rho$ is the inradius. For a convex planar domain, a sharper lower estimate:
			\begin{align*}
				\lambda^2_2 - \lambda^2_1 \ge \frac{3\pi^2}{\delta^2}.
			\end{align*}
		I recall looking at a simple $2$D problem where I fixed a $\lambda^2_n$ and looked at the nodal domain of its eigenfunction. The second eigenvalue of this nodal domain problem was an eigenvalue further along the spectrum past $\lambda^2_n$ (and not $\lambda^2_{n+1}$ as I naively hoped). I need to double check this, but perhaps this will give us bounds on a gap between a subset of eigenvalues?
	\end{enumerate}


















==> trimFig.tex <==
% -------------------------------------------------------------------------------------
%
% Trim a figure: **NEW VERSION**
%  In this new version we hard code the original width of the plot to match an Overture figure.
%  The clipping parameters then denote fractions of this width (width=7.5 in = 19.05 cm)
%
%  \trimPlot{file}{width}{xa}{xb}{ya}{yb}
% Trim a figure and show the bounding box:
%  \trimPlotb{file}{width}{xa}{xb}{ya}{yb}
% 
%  file = name of the graphics file for includegraphics : .eps or pdf or ...
%  width : final width (after trimming) of the figure e.g. 5cm
%  xa,xb,ya,yb : trim this fraction of the width from the left, right, bottom and top
% 
% -----------------------------------------------------------------------------------------
\newlength{\tfwidth}
\newlength{\tfheight}
\newlength{\tfxa}
\newlength{\tfxb}
\newlength{\tfya}
\newlength{\tfyb}
% 
\newcommand{\trimPlotWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
\newcommand{\trimPlotNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% Trim a figure and draw the bounding box 
% Overture figures are 7.5 inches wide (8.5 - .5 -.5) = 19.05 cm
\newcommand{\trimPlotb}[6]{%
\setlength{\tfwidth}{19.05cm}%   % width of un-clipped fig
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfwidth*\real{#5}}%
\setlength{\tfyb}{\tfwidth*\real{#6}}%
% trim=l b r t
\trimPlotWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
% \trimPlotWithBox{#1}{#2}{#3}{#4}{#5}{#6}%
}
% Trim a figure 
% 
\newcommand{\trimPlot}[6]{%
\setlength{\tfwidth}{19.05cm}%   % width of un-clipped fig
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfwidth*\real{#5}}%
\setlength{\tfyb}{\tfwidth*\real{#6}}%
% trim=l b r t
\trimPlotNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% ----------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------
%
% Trim a figure: 
%  \trimFig{file}{width}{xa}{xb}{ya}{yb}
% Trim a figure and show the bounding box:
%  \trimFigb{file}{width}{xa}{xb}{ya}{yb}
% 
%  file = name of the graphics file for includegraphics : .eps or pdf or ...
%  width : final width (after trimming) of the figure e.g. 5cm
%  xa,xb,ya,yb : trim this fraction of the width from the left, right, bottom and top
% 
% -----------------------------------------------------------------------------------------
\newcommand{\trimFigWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
% -----------------------------------------------------------------------------------------
\newcommand{\trimFigNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% ---------- Set height -----
\newcommand{\trimFigHeightWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[height=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
% ---------- Set height -----
\newcommand{\trimFigHeightNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[height=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% Trim a figure and draw the bounding box 
\newcommand{\trimFigb}[6]{%
\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
% trim=l b r t
\trimFigWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% Trim a figure 
% 
\newcommand{\trimFig}[6]{%
\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
% trim=l b r t
\trimFigNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

%%%%%%%%%%%%%% TRIMW : trim and set width %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% THIS VERSION WORKS PROPERLY %%%%%%%%%%%%%%%%%%
%  Thanks to Longfei Li
% New:
% Trim a figure (working) 
%  trims #3 #4 #5 #6 percent of left, right, bottom, top of the original figure
\newsavebox\figBox

\newcommand{\trimw}[6]{%
%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMWB : trim and set width %%%%%%%%%%%%%%%%%%
%%%%%%%%%%   Version of trim that also draws the bounding box %%%%%%%%%%%%
\newcommand{\trimwb}[6]{%
%old: 
%\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
%\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
%new: Longfei 20160727: we should get the size of the original picture:
%\settowidth\tfwidth{\includegraphics{#1}}
%\settoheight\tfheight{\includegraphics{#1}}

%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMH : trim and set height %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% THIS VERSION WORKS PROPERLY %%%%%%%%%%%%%%%%%%
%  Thanks to Longfei Li
% New:
% Trim a figure (working) 
%  trims #3 #4 #5 #6 percent of left, right, bottom, top of the original figure
\newcommand{\trimh}[6]{%
%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigHeightNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMWB : trim and set height %%%%%%%%%%%%%%%%%%
%%%%%%%%%%   Version of trim that also draws the bounding box %%%%%%%%%%%%
\newcommand{\trimhb}[6]{%
%old: 
%\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
%\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
%new: Longfei 20160727: we should get the size of the original picture:
%\settowidth\tfwidth{\includegraphics{#1}}
%\settoheight\tfheight{\includegraphics{#1}}

%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigHeightWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% ----------------------------------------------------------------------------------------------
% 

